New Insights into the Problem of the Surface Gravity Distribution of Cool DA White Dwarfs

We review at length the longstanding problem in the spectroscopic analysis of cool hydrogen-line (DA) white dwarfs (Teff < 13,000 K) where gravities are significantly higher than those found in hotter DA stars. The first solution that has been proposed for this problem is a mild and systematic helium contamination from convective mixing that would mimic the high gravities. We constrain this scenario by determining the helium abundances in six cool DA white dwarfs using high-resolution spectra from the Keck I 10-m telescope. We obtain no detections, with upper limits as low as He/H = 0.04 in some cases. This allows us to put this scenario to rest for good. We also extend our model grid to lower temperatures using improved Stark profiles with non-ideal gas effects from Tremblay & Bergeron and find that the gravity distribution of cool objects remains suspiciously high. Finally, we find that photometric masses are, on average, in agreement with expected values, and that the high-log g problem is so far unique to the spectroscopic approach.

==> README <==
                                                    February 16th, 2010

Dear Dr. Gies,

Please find below the revised electronic version of our paper entitled:

"New Insights into the Problem of the Surface Gravity Distribution of
Cool DA White Dwarfs"

by P.-E. Tremblay, P. Bergeron, J.S. Kalirai, and A. Gianninas, which
was submitted for publication in the Astrophysical Journal.

We would like to thank the referee, Detlev Koester, for a careful
reading of our manuscript and for his constructive comments which have
been taken into account in our revised version, unless otherwise
stated in our response. We describe below the changes made to our
manuscript. We hope these changes will be acceptable to both you and
the referee.

All correspondence should be sent to:

        Pier-Emmanuel Tremblay
        Department of Physics
        University of Montreal
        2900 boul. Edouard-Montpetit
        Montreal, Quebec
        Canada H3T 1J4

        e-mail: tremblay@astro.umontreal.ca
        Phone : (514) 343-6678
        FAX:    (514) 343-2071

Files submitted:

  README      This file
  ms.tex      Manuscript file
  ms.aux      Auxiliary file for cross-references
  tab1.tex    Table 1
  tab1.aux    Auxiliary file for cross-references
  f1.eps      This file and following are Figure files
  f2.eps      (color figure) 
  f3.eps
  f4.eps     
  f5.eps     
  f6.eps     
  f7.eps     
  f8.eps     
  f9.eps     
  f10.eps     
  f11.eps     
  f12.eps     
  f13.eps     (color figure) 
  f14.eps     

========================================================================

We would like to thank the referee, Detlev Koester, for a careful
reading of our manuscript and for his constructive comments which have
been taken into account in our revised version, unless otherwise
stated in our response below. We describe the changes made to our
manuscript in turn:

> 1. Undoubtedly the work of Bergeron et al. (1995) has defined the standard
> MLT version in use up to now. However, the authors could include a
> reference to Koester et al. (1994, A&A 291, L9), who - using a very
> similar method, although with only one object, had arrived at the same
> conclusion. Their choice (ML1/2.0) produces very similar models as
> ML2/0.6.

We added a footnote with a reference to the earlier work of Koester et
al. (1994).

  "Koester et al. (1994) arrived at a similar conclusion with a somewhat 
   equivalent version of the mixing-length theory, ML1/$\alpha=2.0$, 
   although their analysis was based on a single object."

> 2. Koester et al. (2009) also searched ~1800 spectra of the SPY sample for
> DAs with traces of helium, among those a fairly large number below 13000
> K. That sample was the source of the first detection of a helium-rich
> "DA". The search was also negative, but with a much larger detection limit
> than the Keck observations in the current paper. Nevertheless, it is a
> good argument that such objects as GD362 and HS0146+1847 must be very
> rare.

We agree with the referee that this is a further proof that most
massive DA white dwarfs with a temperature slightly below 13,000 K do
not show large helium contamination. We expanded one section of
the text:

  "The peculiar helium-dominated star HS 0146+1847, the hotter
   counterpart of GD 362, was discovered in the SPY sample containing
   more than ~1800 high-resolution spectra; Koester et al. (2009)
   searched this sample for DA stars with traces of helium, including a
   fairly large number with temperatures below 13,000 K. The search was
   also negative, but with a much larger detection limit than provided
   here with our Keck I observations.  Nevertheless, it is an additional
   argument that such objects must be very rare."

> 3. I have another possible explanation for the unsatisfactory fit of He I
> 5875 in GD362. Zuckerman et al. (2007) use the same He Stark broadening
> profiles from Beauchamp (1995). These profiles are somewhat problematic in
> the line centers, since they were calculated on a fixed wavelength scale.
> Because - unlike the hydrogen profiles - the helium profiles shift with
> electron density, the sharp central maximum was missed in many profiles,
> in particular at low electron densities, where the profiles are narrow.
> This can be shown by integrating the profiles over wavelength, which gives
> sometimes values much less than 1.0. While this is totally unimportant
> outside the very narrow core, it has an unfortunate effect when convolving
> the profiles with the Doppler profile (and in my case with neutral
> broadening profiles). If the Stark core is narrow compared to the Doppler
> profile, the resulting profile will have a core, which is much too low at
> the center. Again, outside the Doppler core of the profile this has no
> effect, but in the line core it does.

This is a valid point worth investigating further, although we are a
bit skeptical since this would not explain why the line is predicted
correctly for HS 0146+1847 but not for GD 362. But this issue is
clearly outside the scope of our paper.

> 4. The authors mention the work of Kilic et al. (2008) on GD362, but don't
> use the result. The parallax determined there leads to a mass of 0.74
> Msun, using only the Teff and Woods MRR, but consistent with the higher
> log g. Apparently this seems to favor the Zuckerman et al. (2007) values.

We agree with the referee and this is what we meant to say in the
text. To be more explicit, we now quote the result from Kilic et
al. (2008) at the end of the first paragraph of page 10:

  "The independent mass determination reported by Kilic et al. (2008), 
   M = 0.74 Mo, which is based on a measurement of the trigonometric
   parallax of GD 362, actually favors the solution of Zuckerman et al.,
   but see our discussion below."

> 5. I am slightly worried about the spectroscopic results for G29-38.
> While for the other one object which I can compare (G67-23), the result is
> very similar to the result in BLH05, for G29-38 the result there was
> 11820/8.15 and now is 12200/8.22. The lower value is much closer to what I
> obtain in various attempts, including most recently with models including
> the new T&B Stark profiles. This is one of the brightest ZZ Ceti stars and
> one of the best studied white dwarfs overall. It would be nice if the
> authors could elaborate with a sentence or two, what caused this change.
> If it remains like that, we will need a new empirical determination of the
> ZZ Ceti instability strip (I'm almost sure Montreal is already working on
> that!).

We confirm that the differences observed by the referee for G29-38 are
real and they are the result of our new Stark profiles described in
Tremblay & Bergeron (2009) as well as our new calibration of the
convective efficiency. The implication of these new models on the
location of the ZZ Ceti instability strip, and on the atmospheric
parameters of DA stars in general, is the topic of the PhD thesis of
one of the co-authors, A. Gianninas, and we want to refrain from
discussing these issues here. Our full analysis of over 1200
relatively bright DA white dwarfs from the McCook & Sion catalog is
underway, the results of which should be submitted for publication
during the summer. But briefly, we find that the blue edge of the ZZ
Ceti instability strip is shifted towards higher effective
temperatures more than the red edge, resulting in a wider instability
strip (which remains pure by the way...).

